Res-embedding for Deep Learning Based Click-Through Rate Prediction Modeling

Recently, click-through rate (CTR) prediction models have evolved from shallow methods to deep neural networks. Most deep CTR models follow an Embedding\&MLP paradigm, that is, first mapping discrete id features, e.g. user visited items, into low dimensional vectors with an embedding module, then learn a multi-layer perception (MLP) to fit the target. In this way, embedding module performs as the representative learning and plays a key role in the model performance. However, in many real-world applications, deep CTR model often suffers from poor generalization performance, which is mostly due to the learning of embedding parameters. In this paper, we model user behavior using an interest delay model, study carefully the embedding mechanism, and obtain two important results: (i) We theoretically prove that small aggregation radius of embedding vectors of items which belongs to a same user interest domain will result in good generalization performance of deep CTR model. (ii) Following our theoretical analysis, we design a new embedding structure named res-embedding. In res-embedding module, embedding vector of each item is the sum of two components: (i) a central embedding vector calculated from an item-based interest graph (ii) a residual embedding vector with its scale to be relatively small. Empirical evaluation on several public datasets demonstrates the effectiveness of the proposed res-embedding structure, which brings significant improvement on the model performance.

==> Introduction_wkl.tex <==
\section{Introduction}

In the advertising and recommendation systems, CTR (click-through rate) prediction is a crucial task to decide final ranking of goods that is presented to the consumers. The CTR prediction tasks has attracted a lot of attention and achieved great success, and it has become the cornerstone of advertising and recommendation systems in many large enterprises.

In recent years, thanks to the rapid development of the deep learning, deep learning based methods for CTR prediction task have gained rapid development. Deep CTR prediction model ultilizes historical behaviors of the users and other features to predict the probability that they click on a goods. 
Most deep CTR prediction models follow a similar Embedding\&MLP structure as Figure \ref{fig:mlpemb}: Embedding layer maps each goods and other features to a low dimensional vector. Input features are transformed into the fixed-length vectors through the embedding layer and fed into a MLP(multilayer perceptron) to learn the nonlinear relations among features.
 \begin{figure}[ht]
	\centering
	\includegraphics[scale=0.14]{embedding_MLP.png}
	\caption{The graph of the embedding\&MLP structure.}
	\label{fig:mlpemb}
\end{figure}

There have been many studies to enhance the back-end MLP such as PNN, deep\&wide, DeepFM, DIN. 
%Based on the original MLP, some attempt to integrate higher-order information of features like PNN and DeepFM. Some researches have tried to extract more advanced features based on user behavior sequences. For instance, DIN adaptively obtains the users' interest representation vector based on the historical behavior of a given candidate advertisement. In addition, some also use sequence-based DNN like RNN, GRU and LSTM to model users' historical behaviors in the CTR prediction.
Compared with the quick evolution of back-end MLP, the embedding layer has become an almost inconvertible input of the CTR prediction model. In this paper, we point out the significance of embedding layer and study the influence of embedding layer on the CTR prediction model. Moreover, a novel embedding structure is proposed to improve the generalization performance of CTR prediction model.
%proved that the generalization error of back-end DNN is bounded by the aggregation radius of embedding vectors under the same insterest state and propose residual embedding layer according to this theoretical result.


Due to the mapping mechanism of embedding layer, the input distribution of back-end MLP could be determined by the embedding layer. Refering to the data-dependent generalization theory[], input distribution will influence the generalization of MLP. Therefore, distribution of embedding vectors is vital to promote the generalization of the CTR prediction model. However, in E-commerce scenarios, original embedding layer will bring MLP poor generalization. For example, 
%the distance among embedding vectors can't illustrate the relationship of corresponding goods in the real world. Besides, 
it exists overfitting phenomenon in the training step. Huge goods scale in E-commerce scenarios causes huge scale of the embedding layer. Huge number of parameters of embedding layer will promote the memory ability but may decrease the generalization ability. Moreover, it can be hard for model to learn embedding vectors with high generalization ability only under the supervision of click labels.
%Although some work based on the pretrained embedding mprove preformances of the CTR recently, they don't explain why the performance of CTR prediction task can be improved by minimizing a no-CTR loss function theoretically.

In this paper, we prove that the generalization error of back-end MLP is bounded by the embedding vectors aggregation radius of goods under the same insterest domain. According to the theoretical analysis, a graph-based residual embedding structure is designed to improve the generalization performance of deep CTR model. we define the countable interest hidden state $z\in Z$ and assume that the conditional distribution of embeddding vectors of the items is different under different $z$. The historical behaviors of users are generated based on a sequence of interest state $\tilde{Z}=\{z_1,z_2,...,z_n\},z_i\in Z$. The user's click behaviors in certain time period are determined by the corresponding elements of $\tilde{Z}$. Referring to analysis of robustness and generalization, we prove that the generalization error bound of back-end DNN is determined by the aggregation radius of embedding vectors under the same interest state $z$. 
%In other words, the closer embedding vectors of the Items user clicked in a short term are, the better generalization performance of the DNN model has.
 
In view of this conclusion, Res-embedding structure is proposed to enhance the generalization of MLP. In this structure, the embedding vector of each goods is composed of sum of central embedding vector and residual embedding vector. The goods in the same interest domain shared the similar central embedding vectors and each goods owns unique and low-scale residual embedding vector. Under this structure constraint, the radius of the embedding vectors under the same insterest hidden state is bounded by the scale of the residual embedding. According to theoretical analysis, the generalization error will be bounded by the scale of the residual embedding. When implementing Res-embedding specifically, the most difficult step is to obtain which goods are belong to one insterest state. Due to the assumption that a insterest hidden state $z$ impacts a period of users' click behaviors, we believe the goods appearing commonly in  historical behaviors of the same user are likely in the same insterest state. Therefore, we build a goods graph based on the frequency that the two goods appearing commonly in the shortterm of historical behaviors. For each goods, its final center embedding vector is calculated by fusing the central embedding vectors of itself and its neighboring goods in the graph. This mechanism makes final central embedding vectors of goods in the same interest domain more likely to be closed. We adopted the average, GCN and attention technology as central embedding fusion mechanism.
Based on this embedding structure with deep CTR prediction models, we achieve the performance over that of state-of-the-art deep CTR prediction models with original embedding layer.


%a residual structure to enhance the generalization performance of the embedding layer. In this structure, the embedding vector of one item is the summation of central embedding vector and residual embedding vector. Goods that the same user clicks within short time period shared the same or similar central embeddings, and the residual embedding vectors of different items with small scale are different from each other. We propose an auxiliary loss to train the sharing relationship of central embedding vector.




The main contributions of our paper are listed as follows:
\begin{itemize}
	\item We have theoretically proved that increasing the degree of aggregation of embedding vectors in the same user behavior help decrease the generalization error bound. This may be a direction worth studying for the future to improve the generatlization perfomance of the embedding layer.
	\item Based on our theoretical results, we propose an Res-embedding  structure to enhance the generalization of the embedding vectors. In addition, GCN with several fusion technologies is successfully introduced to integrate similar central embedding vectors.
	\item Our experimental results verify the correctness of our theory and the effectiveness of residual embedding techniques. We observed the influence of clustering property of embedding vectors on the generalization performance of models in visualization experiments. %The proposed approaches have been proved to be able to improve generalization performance in public datasets and Alibaba production datasets.
\end{itemize}

The rest of the paper is organized as follows. The related work is summarized in section 2. Section 3 theoretically analyzes the influence of the distribution of embedding vectors on the generalization performance of MLP. We propose the base residual embedding stucture and its improved version based on GCN in section 4. Our experimental results are shown in section 5 and conclude in section 6. 

